MMS-MSG: A Multi-purpose Multi-Speaker Mixture Signal Generator

The scope of speech enhancement has changed from a monolithic view of single, independent tasks, to a joint processing of complex conversational speech recordings. Training and evaluation of these single tasks requires synthetic data with access to intermediate signals that is as close as possible to the evaluation scenario. As such data often is not available, many works instead use specialized databases for the training of each system component, e.g WSJ0-mix for source separation. We present a Multi-purpose Multi-Speaker Mixture Signal Generator (MMS-MSG) for generating a variety of speech mixture signals based on any speech corpus, ranging from classical anechoic mixtures (e.g., WSJ0-mix) over reverberant mixtures (e.g., SMS-WSJ) to meeting-style data. Its highly modular and flexible structure allows for the simulation of diverse environments and dynamic mixing, while simultaneously enabling an easy extension and modification to generate new scenarios and mixture types. These meetings can be used for prototyping, evaluation, or training purposes. We provide example evaluation data and baseline results for meetings based on the WSJ corpus. Further, we demonstrate the usefulness for realistic scenarios by using MMS-MSG to provide training data for the LibriCSS database.

==> table_learnable_vs_stft.tex <==

\begin{table*}[hbt]
% 
    \sisetup{detect-weight}
	\robustify\bfseries  % https://tex.stackexchange.com/a/573662/148912
    \sisetup{round-precision=2,round-mode=places, table-format = 2.1}
% 	\sisetup{round-precision=2,round-mode=places, table-format = 1.2}
% 
    \centering
    \vspace{-6pt}  % Compensate "\vskip 10pt" from spconf.sty
        \caption{Separation performance of the SepFormer on SMS-WSJ with a learnable and STFT encoder/decoder and varying  encoder shifts/sizes}
    \label{tab:encoder_sizes_anechoic_and_reverberant}
    \begin{tabular}{c c c c S S S S S S S S}
    \toprule
    \multirow{2}{*}{\shortstack[c]{win. \\ size}} & \multirow{2}{*}{\shortstack[c]{latent \\ size}} & \multirow{2}{*}{shift} & \multirow{2}{*}{\shortstack[c]{learnable \\ encoder}} & 
        \multicolumn{4}{c}{anechoic data} & \multicolumn{4}{c}{reverberant data} \\
    \cmidrule(lr){5-8}\cmidrule(lr){9-11}%\cmidrule{7-9}\cmidrule{11-13}
     &  &  &  & 
        {SDR [\si{\decibel}]} & {WDO}&{PESQ} & {WER [\si{\percent}]} & {SDR [\si{\decibel}]} &  {WDO}& {PESQ} &{WER [\si{\percent}]} \\
    \midrule
    16  & 256  & 8 & \cmark & 
        \bfseries 19.13  & \bfseries 0.85483895 &\bfseries 3.43  & \bfseries 10.19  &   % outdoor_clownfish
        8.98 & 0.799359321594 & 1.83 & 36.83 \\           % crucial_minnow
    256 & 256  & 8 & \cmark & 
        16.68 & 0.82759815 &3.11 & 12.36 &  % functional_wallaby
        10.56 & 0.8288679718971252&\bfseries 1.91 & 32.74 \\     % tiny_ox
    256 & 256  & 16 & \cmark & 
        15.27 & 0.8188877105712891 & 3.00 &  15.13 &   % mute_flamingo
        10.23 & 0.8194860219955444 &1.85 & 35.43 \\        % cooing_ermine
    256 & 256  & 64 & \cmark & 
        11.86 &0.8426356315612793 &  2.47 & 26.33 &  % hurt fish
        9.52 & \bfseries 0.8507705926895142 & 1.83 & 37.64\\         % pale_wasp
 \midrule
    16  & 256  & 8 & \xmark & 
        16.74 & 0.7358398986230643 & 2.84 & 13.68 &  % obedient_vicuna
        7.44 & 0.6995357139360081& 1.71 & 51.60\\           % controversial_wildcat
    256 & 256  & 8 & \xmark & 
        15.70 & 0.7924350439190095 & 2.91 & 13.28&   % right_rook
        9.17 & 0.775708516581603  & 1.76 & 35.99\\           % visible_aphid 
    256 & 256  & 16 & \xmark & 
        14.47 & 0.7924365930319872 & 2.69 & 17.98 & % ultimate_amphibian
        \bfseries 10.67 & 0.775707768761923 & 1.90 & \bfseries{29.62} \\   % depressed_ladybug
    256 & 256  & 64 & \xmark & 
        13.52 & 0.7924355352549952 & 2.66 &25.08 &  % steady_galliform
        10.01 & 0.775725939190082 & 1.83 & 36.18 \\        % multiple_leopon
    \bottomrule
    \end{tabular}

\end{table*}

% \begin{table}[hbt]
%     \centering
%         \caption{Separation performance of the Sepformer with a learnable and STFT encoder/decoder and varying  encoder shifts/sizes for reverberant data}
%     \label{tab:encoder_sizes_reverb}
%     \begin{tabular}{c c c|c|c|c|c}
%     win. & emb. & \multirow{2}{*}{shift} & learnable & SDR & PESQ & WER \\
%     size & size &  & encoder & [\si{\decibel}] & &[\si{\percent}] \\
%     \toprule
%     16  & 256  & 8 & \cmark & 
%         \num{8.98} & \num{1.80} &\num{36.83} \\           % crucial_minnow
%     256 & 256  & 8 & \cmark & 
%         \num{10.56} & \bfseries{1.91}& \num{32.74} \\     % tiny_ox
%     256 & 256  & 16 & \cmark & 
%         \num{10.23} & \num{1.85} & \num{35.43} \\        % cooing_ermine
%     256 & 256  & 64 & \cmark & 
%         \num{9.52} & \num{1.83} &  \num{37.64}\\         % pale_wasp
%  \midrule
%     16  & 256  & 8 & \xmark & 
%         \num{7.44} & \num{1.71} & \num{51.60}\\           % controversial_wildcat
%     256 & 256  & 8 & \xmark & 
%         \num{9.17} & \num{1.76} & \num{35.99}\\           % visible_aphid WIP
%     256 & 256  & 16 & \xmark & 
%         \bfseries{10.67} & \num{1.90} & \bfseries{29.62} \\   % depressed_ladybug
%     256 & 256  & 64 & \xmark & 
%         \num{10.01} & \num{1.83} & \num{36.18} \\        % multiple_leopon
%     \end{tabular}
% \end{table}
